Avoiding Materialisation for Guarded Aggregate Queries

Optimising queries with many joins is known to be a hard problem. The explosion of intermediate results as opposed to a much smaller final result poses a serious challenge to modern database management systems (DBMSs). This is particularly glaring in case of analytical queries that join many tables, but ultimately only output comparatively small aggregate information. Analogous problems are faced by graph database systems when processing analytical queries with aggregates on top of complex path queries. In this work, we propose novel optimisation techniques both, on the logical and physical level, that allow us to avoid the materialisation of join results for certain types of aggregate queries. The key to these optimisations is the notion of guardedness, by which we impose restrictions on the occurrence of attributes in GROUP BY clauses and in aggregate expressions. The efficacy of our optimisations is validated through their implementation in Spark SQL and extensive empirical evaluation on various standard benchmarks.

==> expdetailsapp.tex <==
\section{Details of Experimental Setup}
\label{sect:ExperimentalSetup}

We perform the experiments on a machine with two AMD EPYC 75F3 32-Core CPUs and 960 GB RAM.
On top of this, we use a VM with 60 cores running Ubuntu 22.04.2 LTS and Spark SQL (Version 3.5.0).
%
For our experiments, we implement the optimisations presented in Section~\ref{sect:OurSystem} 
and the physical operator from Section~\ref{sect:physicalOpt} natively in Spark SQL. 
%and use its PySpark packaging\footnote{https://anonymous.4open.science/r/spark-4C8C/README.md}%\footnote{\url{https://github.com/arselzer/spark/releases/tag/v3}}. %Our experiments for optimised queries are run on an unmodified installation of Spark but using this modified version of PySpark.
Our experimental setup, including the versions of all dependencies,
is reproducible through a docker-compose environment available at \url{https://github.com/dbai-tuw/spark-eval}. %This makes it possible to reproduce the experiments with only docker-compose as a dependency.
 %used for the experiments is published as a standard python package. Further instructions for running the benchmarks can be found in the README.

In order to import the benchmark databases into Spark SQL, we run a second container with PostgreSQL 16, from where the data is fetched over JDBC.
We configure Spark with 900 GB maximum executor memory and 60 available cores. Off-heap storage (to disk) is disabled in order to avoid performance degradation caused by unexpected use of disk storage for intermediate results. 
In our experiments, we encountered some instances where the excessive memory consumption caused the query to fail. However, these cases exhibited such extreme performance differences that they do not impact the conclusions drawn from our experimental evaluation. Specifically,  queries where Spark SQL failed due to requiring more than 900GB of memory are easily solved by our implementation, using  only a small fraction of the available resources.
%While we do observe cases in our experiments where excess memory consumption leads to failure to answer the query, the performance differences in these cases are so extreme (queries where standard Spark SQL fails due to requiring over 900GB of memory are all easily solvable with our methods) that this does not notably affect the conclusions drawn from our experimental evaluation.  %The number of cores used for execution is varied depending on the concrete experiments.


We evaluate the performance of the optimisation over 5 benchmark datasets 
with different characteristics. As already mentioned before, the problems faced by
graph database systems on analytical queries with aggregates on top of path queries are 
similar to the ones faced by relational database systems in case of 
aggregates on top of joins. Hence, in addition to widely used relational benchmarks 
(JOB, STATS/STATS-CEB, TCP-H), we have also chosen a popular benchmark for graph queries
(SNAP) and one that combines features from relational and graph databases (LSQB):  

\begin{itemize}
    \item The \textit{Join Order Benchmark (JOB)}~\cite{DBLP:journals/pvldb/LeisGMBK015} is a benchmark based on the IMDB real-world data set and a large number of realistic join-aggregation queries featuring many joins and various filtering conditions. It was introduced to evaluate the join ordering problem and evaluate the performance of query optimisers.
    %
    \item The \textit{STATS / STATS-CEB}~\cite{DBLP:journals/pvldb/HanWWZYTZCQPQZL21} benchmark serves a similar purpose as the JOB benchmark but with the explicit addition of joins that do not follow FK/PK relationships (but rather FK/FK to keep with typical usage patterns). %The data is based on anonymised content from Stack Exchange.
    %
    \item \textit{TPC-H}~\cite{tpch} and TPC-DS~\cite{tpcds} are standard benchmarks for relational databases that cover a wide range of complex real-world workloads. {\color{red} In addition, we report performance of our running example query from Example~\ref{exp:median} under the name "TPC-H Ex.1"}. We use scale factor 200 in the generation of the TPC-H data.
    %
    \item The \textit{Large-Scale Subgraph Query Benchmark (LSQB)} \cite{DBLP:conf/sigmod/MhedhbiLKWS21} is a benchmark of 9 graph queries, designed to test the query optimiser and executor of graph databases as well as relational databases. Its schema represents a social network scenario with relations for e.g., persons, posts, and comments. 
    We generate data with scale factor 300 for LSQB.% process of this benchmark.
    %Data generation is based on the LDBC\cite{DBLP:journals/corr/abs-2001-02299} benchmark, a synthetic benchmark which takes care to closely mirror the properties of real-life social networks. The benchmark consists of 11 relations with various scale factors (e.g., 10, 30, 100, 300), as well as 9 queries in various query languages (SQL, Cypher, etc.). 
    \item The  \textit{SNAP (Stanford Network Analysis Project}
    \cite{snapnets}) dataset is commonly used to benchmark queries on graph data (e.g., in \cite{DBLP:journals/pacmmod/0005023}).
%    Most SNAP datasets consist of a single, directed or undirected, edge relation, such as the the US patent citation dataset (cit-Patents), or the Google web graph (web-Google).
In particular, we experiment on the following two popular graphs of various sizes:

\medskip
{\small\hspace{1em}
    \begin{tabular}{c|c|c|c}
%    \toprule
\centering
        \textbf{Graph} & \textbf{Nodes} & \textbf{Edges} & \textbf{(un)directed} \\
        \midrule
         % cit-Patents & 3,774,768 & 16,518,948 & directed \\
         % \hline
         %wiki-topcats & 	1,791,489 & 28,511,807 & directed \\
         %\hline
         web-Google & 875,713 & 5,105,039 & directed \\
         %\hline
         com-DBLP & 317,080 & 1,049,866 & undirected \\
         %\bottomrule
    \end{tabular}
    }
\medskip

For our experiments, we evaluate the performance of basic graph queries, namely path queries requiring 
between 3 and 8 joins (i.e., between 4 and 9 edges) 
and three small tree queries. For example, the path with 3 joins (path-03) 
over the web-Google graph is expressed in SQL as

\medskip

{ \small
\begin{minted}{sql}
    SELECT COUNT(*) FROM
    edge e1, edge e2, edge e3, edge e4
    WHERE e1.toNode = e2.fromNode
     AND  e2.toNode = e3.fromNode
     AND  e3.toNode = e4.fromNode
\end{minted}
}

\medskip

\noindent
These queries can be viewed as counting the number of homomorphisms from certain patterns (i.e., paths and trees in this case). This task has recently gained popularity in graph machine learning where the results of the queries are injected into machine learning models (e.g.,~\cite{DBLP:conf/icml/NguyenM20,DBLP:conf/nips/BarceloGRR21,DBLP:journals/corr/abs-2402-08595,bao2024homomorphismcountsstructuralencodings}).

\end{itemize}
